A Lightweight FPGA-based IDS-ECU Architecture for Automotive CAN

Recent years have seen an exponential rise in complex software-driven functionality in vehicles, leading to a rising number of electronic control units (ECUs), network capabilities, and interfaces. These expanded capabilities also bring-in new planes of vulnerabilities making intrusion detection and management a critical capability; however, this can often result in more ECUs and network elements due to the high computational overheads. In this paper, we present a consolidated ECU architecture incorporating an Intrusion Detection System (IDS) for Automotive Controller Area Network (CAN) along with traditional ECU functionality on an off-the-shelf hybrid FPGA device, with near-zero overhead for the ECU functionality. We propose two quantised multi-layer perceptrons (QMLP's) as isolated IDSs for detecting a range of attack vectors including Denial-of-Service, Fuzzing and Spoofing, which are accelerated using off-the-shelf deep-learning processing unit (DPU) IP block from Xilinx, operating fully transparently to the software on the ECU. The proposed models achieve the state-of-the-art classification accuracy for all the attacks, while we observed a 15x reduction in power consumption when compared against the GPU-based implementation of the same models quantised using Nvidia libraries. We also achieved a 2.3x speed up in per-message processing latency (at 0.24 ms from the arrival of a CAN message) to meet the strict end-to-end latency on critical CAN nodes and a 2.6x reduction in power consumption for inference when compared to the state-of-the-art IDS models on embedded IDS and loosely coupled IDS accelerators (GPUs) discussed in the literature.

==> relatedworks.tex <==
\section{Related Works} \label{rel_work}



==> tables/CNN.tex <==
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.5}
\begingroup
\begin{table}[h]\scriptsize
\begin{tabular}{lcccc}
\hline
                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Throughput\\ GOps/Sec\end{tabular}}           & \textbf{\begin{tabular}[c]{@{}c@{}}Performance \\ Density\\ GOps/KLUTs\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Precision\\ Fixed-Point\end{tabular}}           & \textbf{\begin{tabular}[c]{@{}c@{}}Frequency\\ MHz\end{tabular}}               \\ \hline
\multicolumn{1}{l|}{\textbf{AlexNet}} & 1200                                                                             & 5.38                                                                                 & 16 bits=8,8                                                                        & 166                                                                            \\ \cline{1-1}
\multicolumn{1}{l|}{\textbf{VGG-16}}  & 1025                                                                             & 4.60                                                                                 & 16 bits=8,8                                                                        & 166                                                                            \\ \hline
                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Execution\\ Kilo Cycles \\ (EC)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Memory\\ Kilo Cycles \\ (MC)\end{tabular}}        & \textbf{\begin{tabular}[c]{@{}c@{}}Theoretical\\ Kilo Cycles \\ (TC)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Pipeline \\ Rate\\ (EC+MC)/TC\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\textbf{AlexNet}} & 1096                                                                             & 112                                                                                  & 856                                                                                & 1.45                                                                           \\ \cline{1-1}
\multicolumn{1}{l|}{\textbf{VGG-16}}  & 7046                                                                             & 431                                                                                  & 5149                                                                               & 1.44                                                                           \\ \hline
\end{tabular}
\caption{The table lists the Execution Cycles (EC), Memory Cycles (MC) and Theoretical Cycles (TC) required by our overlay to process various networks. The pipeline rate (PR) to process each network is also reported. }
\label{tab:scale_cnn}
\end{table}
\endgroup

==> tables/resr_utilisation.tex <==
\renewcommand{\arraystretch}{1.5}
\begin{table}[]
\centering
\begin{tabular}{cccc}
\hline
\textbf{Method}                        & \textbf{Adders}   & \textbf{Freq.(MHz)} & \textbf{Slices} \\ \hline
\multicolumn{1}{c|}{\textbf{FCBT}~\cite{zhuo2007high}}     & 2                 & 170                 & 2859            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{DSA}~\cite{zhuo2007high}}      & 2                 & 142                 & 2215            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{SSA}~\cite{zhuo2007high}}      & 1                 & 165                 & 1804            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{DB}~\cite{tai2011accelerating}}       & 1                 & 188                 & 1749            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{MFPA}~\cite{huang2012modular}}     & 5                 & 207                 & 4491            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{AeMFPA}~\cite{huang2012modular}}   & 2                 & 204                 & 3130            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{Ae$^2$MFPA}~\cite{huang2012modular}}   & 2                 & 144                 & 3737            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{SBM}~\cite{tang2019resource}}      & 1                 & 278                 & 1670            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{TreeNet}} & \textbf{36 (FxPt)} & \textbf{200}        & \textbf{5854}   \\ \hline
\end{tabular}
\caption{Table compares the slice consumption of TreeNet along the operating frequency with other works.}
\label{tab:adder-table}
\end{table}

==> tables/util_improv.tex <==
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}
\begin{table}[]\scriptsize
\centering
\begin{tabular}{l|cccccccccccc|}
\cline{2-13}
                                   & \multicolumn{3}{c|}{\textbf{3 x 3}} & \multicolumn{3}{c|}{\textbf{5 x 5}} & \multicolumn{3}{c|}{\textbf{7 x 7}} & \multicolumn{3}{c|}{\textbf{9 x 9}} \\ \cline{2-13} 
\multicolumn{1}{c|}{}              & LUT        & FF         & RAM       & LUT        & FF         & RAM       & LUT        & FF         & RAM       & LUT        & FF         & RAM       \\ \hline
\multicolumn{1}{|l|}{\textbf{1}}   & 2.5x       & 2.1x       & 1.3x      & 2.2x       & 2.2x       & 1.3x      & 2.4x       & 2.8x       & 1.6x      & 2.2x       & 2.6x       & 1.4x      \\
\multicolumn{1}{|l|}{\textbf{2}}   & 2.3x       & 1.9x       & 1.2x      & 1.9x       & 1.9x       & 1.2x      & 2.2x       & 2.4x       & 1.5x      & 2.0x       & 2.1x       & 1.3x      \\
\multicolumn{1}{|l|}{\textbf{4}}   & 2.0x       & 1.9x       & 0.9x      & 1.8x       & 1.9x       & 0.9x      & 2.1x       & 2.4x       & 1.2x      & 1.8x       & 1.8x       & 1.1x      \\
\multicolumn{1}{|l|}{\textbf{8}}   & 1.9x       & 2.0x       & 1.1x      & 1.9x       & 2.1x       & 1.2x      & 2.3x       & 2.3x       & 1.6x      & 2.2x       & 1.9x       & 1.5x      \\
\multicolumn{1}{|l|}{\textbf{16}}  & 2.0x       & 2.2x       & 1.2x      & 1.9x       & 2.3x       & 1.5x      & 2.4x       & 2.5x       & 2.0x      & 2.5x       & 2.3x       & 2.1x      \\
\multicolumn{1}{|l|}{\textbf{32}}  & 2.0x       & 2.3x       & 1.1x      & 1.8x       & 2.5x       & 1.5x      & 2.3x       & 2.7x       & 1.9x      & 1.7x       & 1.7x       & 2.2x      \\
\multicolumn{1}{|l|}{\textbf{64}}  & 2.2x       & 2.5x       & 1.1x      & 1.9x       & 2.7x       & 1.5x      & 2.2x       & 2.5x       & 1.9x      & 2.0x       & 2.0x       & 2.2x      \\
\multicolumn{1}{|l|}{\textbf{128}} & 2.2x       & 2.6x       & 1.1x      & 2.0x       & 2.7x       & 1.5x      & 2.2x       & 2.5x       & 1.9x      & 2.1x       & 2.2x       & 2.3x      \\
\multicolumn{1}{|l|}{\textbf{256}} & 2.3x       & 2.7x       & 1.1x      & 2.1x       & 2.7x       & 1.5x      & 2.3x       & 2.5x       & 2.0x      & 2.1x       & 2.2x       & 2.4x      \\
\multicolumn{1}{|l|}{\textbf{512}} & 2.7x       & 2.9x       & 1.1x      & 2.4x       & 2.1x       & 1.5x      & 2.6x       & 3.0x       & 2.0x      & 3.4x       & 3.3x       & 2.4x      \\ \hline
\end{tabular}
\caption{Absolute resource numbers for the presented approach.}
\end{table}

==> tables/utilization.tex <==
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}
\begin{table*}[]\scriptsize
\centering
\begin{tabular}{cccccccccccccl}
\multicolumn{13}{c}{\textbf{(a) Our Work}}                                                                                                                                                                                                                                                                                                           &  \\ \cline{1-13}
\multicolumn{1}{|c|}{\textbf{Replications}} & \multicolumn{3}{c|}{\textbf{3 x 3}}                                      & \multicolumn{3}{c|}{\textbf{5 x 5}}                                      & \multicolumn{3}{c|}{\textbf{7 x 7}}                                    & \multicolumn{3}{c|}{\textbf{9 x 9}}                                     &  \\ \cline{1-13}
\multicolumn{1}{|c|}{}                      & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM} & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}  &  \\ \cline{2-13}
\multicolumn{1}{|c|}{1}                     & 167                  & 299                  & \multicolumn{1}{c|}{3}     & 270                  & 410                  & \multicolumn{1}{c|}{4.5}   & 327                  & 446                  & \multicolumn{1}{c|}{5}   & 459                  & 637                  & \multicolumn{1}{c|}{7}    &  \\
\multicolumn{1}{|c|}{2}                     & 195                  & 371                  & \multicolumn{1}{c|}{4}     & 324                  & 522                  & \multicolumn{1}{c|}{5.5}   & 375                  & 592                  & \multicolumn{1}{c|}{6}   & 551                  & 887                  & \multicolumn{1}{c|}{8}    &  \\
\multicolumn{1}{|c|}{4}                     & 268                  & 514                  & \multicolumn{1}{c|}{5.5}   & 417                  & 697                  & \multicolumn{1}{c|}{7.5}   & 454                  & 785                  & \multicolumn{1}{c|}{7}   & 676                  & 1272                 & \multicolumn{1}{c|}{10}   &  \\
\multicolumn{1}{|c|}{8}                     & 414                  & 798                  & \multicolumn{1}{c|}{9}     & 610                  & 1044                 & \multicolumn{1}{c|}{11}    & 653                  & 1204                 & \multicolumn{1}{c|}{11}  & 843                  & 1771                 & \multicolumn{1}{c|}{14}   &  \\
\multicolumn{1}{|c|}{16}                    & 681                  & 1363                 & \multicolumn{1}{c|}{16}    & 981                  & 1737                 & \multicolumn{1}{c|}{18}    & 1017                 & 2023                 & \multicolumn{1}{c|}{18}  & 1209                 & 2717                 & \multicolumn{1}{c|}{21}   &  \\
\multicolumn{1}{|c|}{32}                    & 1220                 & 2489                 & \multicolumn{1}{c|}{30.5}  & 1708                 & 3127                 & \multicolumn{1}{c|}{32}    & 1734                 & 3659                 & \multicolumn{1}{c|}{32}  & 2740                 & 6851                 & \multicolumn{1}{c|}{35}   &  \\
\multicolumn{1}{|c|}{64}                    & 2133                 & 4757                 & \multicolumn{1}{c|}{59}    & 3154                 & 5897                 & \multicolumn{1}{c|}{60.5}  & 3425                 & 8064                 & \multicolumn{1}{c|}{61}  & 4485                 & 11681                & \multicolumn{1}{c|}{64}   &  \\
\multicolumn{1}{|c|}{128}                   & 4392                 & 9344                 & \multicolumn{1}{c|}{116}   & 6226                 & 12100                & \multicolumn{1}{c|}{117.5} & 6839                 & 16037                & \multicolumn{1}{c|}{118} & 8458                 & 22210                & \multicolumn{1}{c|}{120}  &  \\
\multicolumn{1}{|c|}{256}                   & 8964                 & 18823                & \multicolumn{1}{c|}{229.5} & 12407                & 24716                & \multicolumn{1}{c|}{231.5} & 13722                & 32998                & \multicolumn{1}{c|}{231} & 17200                & 45615                & \multicolumn{1}{c|}{234}  &  \\
\multicolumn{1}{|c|}{512}                   & 15526                & 36308                & \multicolumn{1}{c|}{457}   & 21916                & 46210                & \multicolumn{1}{c|}{459}   & 24938                & 65388                & \multicolumn{1}{c|}{459} & 21816                & 60139                & \multicolumn{1}{c|}{462}  &  \\ \cline{1-13}
\multicolumn{1}{l}{}                        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}      &  \\
\multicolumn{13}{c}{\textbf{(b) FPGA 2018 }}                                                                                                                                                                                                                                                                                                 &  \\ \cline{1-13}
\multicolumn{1}{|c|}{\textbf{Replications}} & \multicolumn{3}{c|}{\textbf{3 x 3}}                                      & \multicolumn{3}{c|}{\textbf{5 x 5}}                                      & \multicolumn{3}{c|}{\textbf{7 x 7}}                                    & \multicolumn{3}{c|}{\textbf{9 x 9}}                                     &  \\ \cline{1-13}
\multicolumn{1}{|c|}{}                      & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUTs                 & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM} & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}  &  \\ \cline{2-13}
\multicolumn{1}{|c|}{1}                     & 425                  & 631                  & \multicolumn{1}{c|}{4}     & 602                  & 917                  & \multicolumn{1}{c|}{6}     & 805                  & 1278                 & \multicolumn{1}{c|}{8}   & 1040                 & 1695                 & \multicolumn{1}{c|}{10}   &  \\
\multicolumn{1}{|c|}{2}                     & 461                  & 704                  & \multicolumn{1}{c|}{5}     & 638                  & 1032                 & \multicolumn{1}{c|}{7}     & 859                  & 1428                 & \multicolumn{1}{c|}{9}   & 1107                 & 1891                 & \multicolumn{1}{c|}{11}   &  \\
\multicolumn{1}{|c|}{4}                     & 560                  & 990                  & \multicolumn{1}{c|}{5}     & 763                  & 1366                 & \multicolumn{1}{c|}{7}     & 996                  & 1952                 & \multicolumn{1}{c|}{9}   & 1264                 & 2377                 & \multicolumn{1}{c|}{11}   &  \\
\multicolumn{1}{|c|}{8}                     & 823                  & 1632                 & \multicolumn{1}{c|}{10}    & 1158                 & 2252                 & \multicolumn{1}{c|}{14}    & 1528                 & 2856                 & \multicolumn{1}{c|}{18}  & 1911                 & 3484                 & \multicolumn{1}{c|}{22}   &  \\
\multicolumn{1}{|c|}{16}                    & 1379                 & 3017                 & \multicolumn{1}{c|}{20}    & 1925                 & 4121                 & \multicolumn{1}{c|}{28}    & 2489                 & 5231                 & \multicolumn{1}{c|}{36}  & 3059                 & 6354                 & \multicolumn{1}{c|}{44}   &  \\
\multicolumn{1}{|c|}{32}                    & 2444                 & 5919                 & \multicolumn{1}{c|}{35}    & 3216                 & 8070                 & \multicolumn{1}{c|}{49}    & 3997                 & 10176                & \multicolumn{1}{c|}{63}  & 4742                 & 12284                & \multicolumn{1}{c|}{77}   &  \\
\multicolumn{1}{|c|}{64}                    & 4826                 & 11967                & \multicolumn{1}{c|}{65}    & 6265                 & 16119                & \multicolumn{1}{c|}{91}    & 7711                 & 20290                & \multicolumn{1}{c|}{117} & 9218                 & 24465                & \multicolumn{1}{c|}{143}  &  \\
\multicolumn{1}{|c|}{128}                   & 10001                & 24661                & \multicolumn{1}{c|}{130}   & 12747                & 32879                & \multicolumn{1}{c|}{182}   & 15494                & 41194                & \multicolumn{1}{c|}{234} & 18306                & 49486                & \multicolumn{1}{c|}{286}  &  \\
\multicolumn{1}{|c|}{256}                   & 20704                & 51117                & \multicolumn{1}{c|}{260}   & 26262                & 67636                & \multicolumn{1}{c|}{364}   & 31603                & 83955                & \multicolumn{1}{c|}{468} & 37062                & 100310               & \multicolumn{1}{c|}{572}  &  \\
\multicolumn{1}{|c|}{512}                   & 43360                & 106385               & \multicolumn{1}{c|}{515}   & 54097                & 100000               & \multicolumn{1}{c|}{721}   & 64928                & 200000               & \multicolumn{1}{c|}{927} & 75862                & 204114               & \multicolumn{1}{c|}{1133} &  \\ \cline{1-13}
\end{tabular}
\caption{Absolute resource numbers for the presented approach.}
\end{table*}
